Local Algebraic Effect Theories

Algebraic effects are computational effects that can be described with a set of basic operations and equations between them. As many interesting effect handlers do not respect these equations, most approaches assume a trivial theory, sacrificing both reasoning power and safety. We present an alternative approach where the type system tracks equations that are observed in subparts of the program, yielding a sound and flexible logic, and paving a way for practical optimizations and reasoning tools.

==> Figures/logic_semantics.tex <==
% !TeX root = ../main.tex
% chktex-file 1
% chktex-file 46

\newcommand{\etaG}{{\rel_\ctx}}
$\sem{\varphi}$ is notation for $\sem{\ljudgement{\ctx}{\hypo}{\varphi}}$

